Z3RO Precoder Canceling Nonlinear Power Amplifier Distortion in Large Array Systems

Large array-based transmission uses the combination of a massive number of antenna elements and clever precoder designs to achieve array gain and spatially multiplex different users. These precoders require linear front-ends, and more specifically linear power amplifiers (PAs). However, this reduces energy efficiency since PAs are most efficient close to saturation, where they generate most nonlinear distortion. Moreover, the use of conventional precoders, such as \gls{mrt}, induces a coherent combining of distortion at the user location, degrading the signal quality. In this work, a linear precoder is proposed that allows working close to saturation while canceling the coherent combining of the third order nonlinear \gls{pa} distortion at the user location. In contrast to other solutions, the zero third-order distortion (Z3RO) precoder does not require prior knowledge of the signal statistics and the PA model. The design consists of saturating a single or a few antennas on purpose together with an opposite phase shift to compensate for the distortion of all other antennas. The resulting array gain penalty becomes negligible as the number of base station antennas grows large.

==> array_gain.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.9,0.05)},
  anchor=south east,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Number of antennas \(\displaystyle M\)},
xmin=1, xmax=127,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Array gain [dB]},
ymin=0, ymax=22.0380372095596,
ytick style={color=black}
]
\addplot [semithick, black]
table {%
1 0
2 3.01029995663981
3 4.77121254719662
4 6.02059991327962
5 6.98970004336019
6 7.78151250383644
7 8.45098040014257
8 9.03089986991944
9 9.54242509439325
10 10
11 10.4139268515823
12 10.7918124604762
13 11.1394335230684
14 11.4612803567824
15 11.7609125905568
16 12.0411998265592
17 12.3044892137827
18 12.5527250510331
19 12.7875360095283
20 13.0102999566398
21 13.2221929473392
22 13.4242268082221
23 13.6172783601759
24 13.8021124171161
25 13.9794000867204
26 14.1497334797082
27 14.3136376415899
28 14.4715803134222
29 14.6239799789896
30 14.7712125471966
31 14.9136169383427
32 15.0514997831991
33 15.1851393987789
34 15.3147891704226
35 15.4406804435028
36 15.5630250076729
37 15.6820172406699
38 15.7978359661681
39 15.910646070265
40 16.0205999132796
41 16.1278385671974
42 16.232492903979
43 16.3346845557959
44 16.4345267648619
45 16.5321251377534
46 16.6275783168157
47 16.7209785793572
48 16.8124123737559
49 16.9019608002851
50 16.9897000433602
51 17.0757017609794
52 17.160033436348
53 17.2427586960079
54 17.3239375982297
55 17.4036268949424
56 17.481880270062
57 17.5587485567249
58 17.6342799356294
59 17.7085201164214
60 17.7815125038364
61 17.8532983501077
62 17.9239168949825
63 17.9934054945358
64 18.0617997398389
65 18.1291335664286
66 18.1954393554187
67 18.2607480270083
68 18.3250891270624
69 18.3884909073726
70 18.4509804001426
71 18.5125834871908
72 18.5733249643127
73 18.6332286012046
74 18.6923171973098
75 18.750612633917
76 18.8081359228079
77 18.8649072517248
78 18.9209460269048
79 18.9762709129044
80 19.0308998699194
81 19.0848501887865
82 19.1381385238372
83 19.1907809237607
84 19.2427928606188
85 19.2941892571429
86 19.3449845124357
87 19.3951925261862
88 19.4448267215017
89 19.4939000664491
90 19.5424250943932
91 19.5904139232109
92 19.6378782734556
93 19.6848294855393
94 19.731278535997
95 19.7772360528885
96 19.8227123303957
97 19.8677173426624
98 19.9122607569249
99 19.9563519459755
100 20
101 20.0432137378264
102 20.0860017176192
103 20.1283722470517
104 20.1703333929878
105 20.2118929906994
106 20.2530586526477
107 20.2938377768521
108 20.3342375548695
109 20.3742649794062
110 20.4139268515823
111 20.4532297878666
112 20.4921802267018
113 20.5307844348342
114 20.5690485133647
115 20.6069784035361
116 20.6445798922692
117 20.6818586174616
118 20.7188200730613
119 20.7554696139253
120 20.7918124604762
121 20.8278537031645
122 20.8635983067475
123 20.899051114394
124 20.9342168516224
125 20.9691001300806
126 21.0037054511756
127 21.0380372095596
};
\addlegendentry{MRT}
\addplot [semithick, blue, dashed]
table {%
1 -inf
2 -inf
3 -8.16223827461591
4 -3.20875118897935
5 -0.492668096960007
6 1.35452707113651
7 2.74377749477986
8 3.85206307504924
9 4.77121254719662
10 5.55477458751009
11 6.23660277237828
12 6.83941058335455
13 7.37914969106245
14 7.86743651511726
15 8.31298355794006
16 8.72248714008608
17 9.10120122142502
18 9.45332139635319
19 9.78224955660574
20 10.0907810065403
21 10.381239717662
22 10.6555780200622
23 10.9154513616438
24 11.1622752414116
25 11.3972691717331
26 11.6214910518148
27 11.8358643505565
28 12.0411998265592
29 12.2382130483092
30 12.4275386501815
31 12.6097420259022
32 12.7853289915816
33 12.9547538260848
34 13.1184260042454
35 13.276715869245
36 13.4299594380776
37 13.5784624939671
38 13.7225040887182
39 13.8623395539774
40 13.9982031015701
41 14.1303100782514
42 14.2588589284181
43 14.3840329089161
44 14.5060015924979
45 14.6249221903619
46 14.7409407192195
47 14.8541930342663
48 14.964805746087
49 15.0728970367613
50 15.1785773881517
51 15.2819502334469
52 15.3831125414427
53 15.482155341704
54 15.5791641976285
55 15.6742196334783
56 15.7673975206395
57 15.858769427684
58 15.9484029382189
59 16.0363619400088
60 16.1227068884246
61 16.2074950469001
62 16.2907807067582
63 16.3726153884897
64 16.4530480263284
65 16.5321251377534
66 16.6098909793709
67 16.6863876904629
68 16.7616554253556
69 16.8357324756317
70 16.9086553831075
71 16.9804590443965
72 17.0511768078003
73 17.1208405631898
74 17.1894808254763
75 17.2571268122116
76 17.3238065158053
77 17.3895467708001
78 17.4543733166039
79 17.5183108560428
80 17.5813831100627
81 17.643612868879
82 17.7050220398482
83 17.765631692308
84 17.8254620996153
85 17.8845327785865
86 17.9428625265322
87 18.000469456059
88 18.0573710277976
89 18.1135840812039
90 18.1691248635666
91 18.2240090573463
92 18.2782518059584
93 18.3318677381051
94 18.3848709907539
95 18.4372752308507
96 18.4890936758507
97 18.5403391131435
98 18.5910239184422
99 18.6411600732029
100 18.6907591811347
101 18.7398324838567
102 18.7883908757534
103 18.8364449180791
104 18.884004852354
105 18.9310806130959
106 18.9776818399259
107 19.0238178890842
108 19.0694978443914
109 19.1147305276855
110 19.1595245087653
111 19.2038881148672
112 19.2478294397026
113 19.2913563520787
114 19.3344765041259
115 19.3771973391539
116 19.4195260991551
117 19.4614698319754
118 19.5030353981689
119 19.5442294775534
120 19.5850585754825
121 19.6255290288482
122 19.6656470118289
123 19.7054185413936
124 19.7448494825773
125 19.7839455535361
126 19.8227123303957
127 19.8611552519002
};
\addlegendentry{$M_{s}=1$}
\addplot [semithick, red, dashed]
table {%
1 -60
2 -60
3 -60
4 -inf
5 -10.4657801685519
6 -5.1519383179761
7 -2.20727630106629
8 -0.198451232339538
9 1.31289687144841
10 2.51763185967981
11 3.51547206342299
12 4.36482702777632
13 5.1027308627902
14 5.75407745141967
15 6.33636997334793
16 6.86236303168905
17 7.34162559774777
18 7.78151250383644
19 8.18779346309105
20 8.5650745441499
21 8.9170889473673
22 9.24690272901809
23 9.5570635829308
24 9.84971053999437
25 10.1266562496208
26 10.3894496477023
27 10.6394243472638
28 10.8777364717571
29 11.1053945699677
30 11.3232835145799
31 11.5321837752448
32 11.7327870967259
33 11.9257093550715
34 12.1115011780648
35 12.2906567792269
36 12.463621352993
37 12.6307973024464
38 12.7925495132456
39 12.949209843233
40 13.1010809631802
41 13.2484396576577
42 13.3915396743019
43 13.5306141933958
44 13.665877976702
45 13.7975292441058
46 13.9257513182836
47 14.0507140708625
48 14.1725751980514
49 14.2914813492393
50 14.4075691283729
51 14.5209659848889
52 14.6317910084546
53 14.7401556396787
54 14.8461643071963
55 14.9499150000694
56 15.0514997831991
57 15.1510052624068
58 15.248513004949
59 15.3440999204785
60 15.4378386068213
61 15.5297976643849
62 15.620041982542
63 15.708633000926
64 15.7956289482214
65 15.8810850607296
66 15.9650537827246
67 16.0475849503849
68 16.1287259608852
69 16.2085219280586
70 16.2870158258848
71 16.3642486209267
72 16.4402593947175
73 16.5150854569973
74 16.5887624506069
75 16.6613244487612
76 16.732804045358
77 16.8032324389076
78 16.8726395106172
79 16.9410538971094
80 17.0085030582099
81 17.0750133402001
82 17.1406100348912
83 17.2053174348482
84 17.2691588850579
85 17.3321568313125
86 17.3943328655559
87 17.4557077684171
88 17.5163015491377
89 17.5761334830819
90 17.6352221470018
91 17.6935854522178
92 17.7512406758593
93 17.808204490299
94 17.8644929909062
95 17.9201217222312
96 17.9751057027269
97 18.0294594481024
98 18.0831969934011
99 18.1363319138835
100 18.1888773447915
101 18.2408460000667
102 18.2922501900867
103 18.3431018384809
104 18.3934124980825
105 18.4431933660697
106 18.4924552983438
107 18.5412088231908
108 18.5894641542683
109 18.6372312029579
110 18.6845195901181
111 18.7313386572749
112 18.7776974772793
113 18.8236048644636
114 18.8690693843238
115 18.9140993627541
116 18.9587028948587
117 19.0028878533634
118 19.0466618966486
119 19.0900324764241
120 19.1330068450644
121 19.1755920626227
122 19.2177950035399
123 19.2596223630644
124 19.301080663398
125 19.3421762595808
126 19.3829153451295
127 19.4233039574403
};
\addlegendentry{$M_{s}=2$}
\addplot [semithick, green!50!black, dashed]
table {%
1 -60
2 -60
3 -60
4 -60
5 -60
6 -60
7 -60
8 -0.198451232339538
9 1.01383589567915
10 2.00939586091242
11 2.8543193070262
12 3.58824026341124
13 4.23686434169979
14 4.81784395101974
15 5.34384085388949
16 5.82425416152208
17 6.26625735806473
18 6.67545220043624
19 7.05629810286127
20 7.41240380813627
21 7.74673128801175
22 8.06174184668455
23 8.35950307844225
24 8.64176865330889
25 8.91003883071186
26 9.16560704045837
27 9.40959621768283
28 9.6429874865252
29 9.86664305053084
30 10.0813246410959
31 10.2877085208111
32 10.4863977866493
33 10.6779325363373
34 10.8627983286018
35 11.0414332698992
36 11.21423398691
37 11.3815606886736
38 11.5437414799812
39 11.7010760551113
40 11.8538388757441
41 12.0022819171332
42 12.1466370510436
43 12.287118121605
44 12.4239227603566
45 12.5572339788223
46 12.6872215705365
47 12.8140433492236
48 12.9378462455672
49 13.0587672815027
50 13.1769344380732
51 13.2924674304917
52 13.4054784020561
53 13.516072546892
54 13.6243486700991
55 13.7303996926946
56 13.8343131077477
57 13.9361713932542
58 14.0360523865762
59 14.1340296246568
60 14.2301726536916
61 14.3245473114855
62 14.4172159853316
63 14.5082378479117
64 14.5976690734257
65 14.6855630359033
66 14.7719704914275
67 14.8569397458118
68 14.9405168090975
69 15.0227455380954
70 15.1036677680626
71 15.1833234344914
72 15.2617506858872
73 15.3389859883224
74 15.4150642224746
75 15.4900187737867
76 15.5638816163252
77 15.6366833908567
78 15.7084534776144
79 15.7792200641804
80 15.8490102088722
81 15.9178498999848
82 15.9857641112093
83 16.0527768535191
84 16.1189112237913
85 16.1841894504047
86 16.248632936038
87 16.3122622978715
88 16.3750974053778
89 16.4371574158743
90 16.4984608079923
91 16.5590254132094
92 16.6188684455763
93 16.6780065297613
94 16.7364557275245
95 16.7942315627271
96 16.8513490449705
97 16.9078226919544
98 16.9636665506376
99 17.0188942172746
100 17.0735188564021
101 17.1275532188382
102 17.1810096587559
103 17.2339001498878
104 17.2862363009139
105 17.3380293700813
106 17.3892902791018
107 17.4400296263686
108 17.4902576995335
109 17.5399844874791
110 17.5892196917222
111 17.6379727372801
112 17.6862527830286
113 17.7340687315822
114 17.7814292387202
115 17.8283427223857
116 17.8748173712783
117 17.9208611530642
118 17.9664818222229
119 18.0116869275493
120 18.0564838193305
121 18.1008796562122
122 18.1448814117729
123 18.1884958808178
124 18.23172968541
125 18.2745892806483
126 18.3170809602082
127 18.3592108616536
};
\addlegendentry{$M_{s}=4$}
\end{axis}

\end{tikzpicture}

